Multi-Dialect Vietnamese: Task, Dataset, Baseline Models and Challenges

Vietnamese, a low-resource language, is typically categorized into three primary dialect groups that belong to Northern, Central, and Southern Vietnam. However, each province within these regions exhibits its own distinct pronunciation variations. Despite the existence of various speech recognition datasets, none of them has provided a fine-grained classification of the 63 dialects specific to individual provinces of Vietnam. To address this gap, we introduce Vietnamese Multi-Dialect (ViMD) dataset, a novel comprehensive dataset capturing the rich diversity of 63 provincial dialects spoken across Vietnam. Our dataset comprises 102.56 hours of audio, consisting of approximately 19,000 utterances, and the associated transcripts contain over 1.2 million words. To provide benchmarks and simultaneously demonstrate the challenges of our dataset, we fine-tune state-of-the-art pre-trained models for two downstream tasks: (1) Dialect identification and (2) Speech recognition. The empirical results suggest two implications including the influence of geographical factors on dialects, and the constraints of current approaches in speech recognition tasks involving multi-dialect speech data. Our dataset is available for research purposes.

==> Main_Section/4-Method.tex <==
\section{Baseline Models}

Recent progress in speech recognition has been facilitated by the emergence of novel architectures and techniques, such as wav2vec 2.0, XLSR, and Whisper. These models have garnered attention due to their innovative methodologies and promising performance. We are employing these models for the purpose of dataset assessment and evaluation.

\subsection{wav2vec 2.0}

\textbf{wav2vec 2.0} \citep{wav2vec2} is a state-of-the-art self-supervised model for speech processing, featuring a multi-layer CNN for feature extraction, a transformer-based encoder for contextual modeling, and a quantization module for efficient storage and inference. During training, raw audio is mapped to speech representations via the CNN and transformer, which are then quantized and used as targets in a contrastive task to learn robust features. Subsequently, the model is fine-tuned on labeled speech data using CTC loss \citep{ctc} for accurate transcription. Across ASR benchmarks, wav2vec 2.0 has demonstrated superior performance, outperforming prior approaches in accuracy and generalization.

\subsection{XLSR and XLS-R}

\textbf{XLSR} (Cross-lingual Speech Recognition) \citep{xlsr}, notably XLSR-53, extends the capabilities of wav2vec 2.0 to facilitate cross-lingual transfer learning, addressing multi-language speech recognition challenges with limited labeled data. Incorporating a shared quantizer for pre-training on diverse multilingual corpora, XLSR enables extraction of language-agnostic representations. Fine-tuning on target language data adapts XLSR to specific linguistic characteristics.

\textbf{XLS-R} \citep{xls-r}, in addition, is an enhanced version, offering variants up to 2 billion parameters and pre-training on 128 languages, surpassing XLSR-53's coverage.

\subsection{Whisper}
\textbf{Whisper} \citep{whisper} is an advanced ASR system released by OpenAI, leverages self-supervised learning on vast unlabeled multilingual speech data. At its core, Whisper consists of a sequence of transformer-based sequence-to-sequence models integrated with an attention mechanism \citep{attention}. Trained on a corpus of approximately 680,000 hours of speech, Whisper employs multi-task learning, encompassing multilingual ASR, speech translation, language identification, and timestamp prediction. The versatility of Whisper allows seamless transfer to existing datasets without explicit supervision, positioning it as a groundbreaking ASR solution for diverse languages. Operationally, the encoder initially module processes Mel Spectrogram, obtained by converting raw audio, to produce audio features. The decoder then utilizes these audio features along with an additional prompt token sequence to generate audio transcripts.
